Dynamic Time Slot Allocation Algorithm for Quadcopter Swarms

A swarm of quadcopters can perform cooperative tasks, such as monitoring of a large area, more efficiently than a single one. However, to be able to successfully work together, the quadcopters must be aware of the position of the other swarm members, especially to avoid collisions. A quadcopter can share its own position by transmitting it via radio waves and in order to allow multiple quadcopters to communicate effectively, a decentralized channel access protocol is essential. We propose a new dynamic channel access protocol, called Dynamic time slot allocation (DTSA), where the quadcopters share the total channel access time in a non-periodic and decentralized manner. Quadcopters with higher communication demands occupy more time slots than less active ones. Our dynamic approach allows the agents to adapt to changing swarm situations and therefore to act efficiently, as compared to the state-of-the-art periodic channel access protocol, time division multiple access (TDMA). Along with simulations, we also do experiments using real Crazyflie quadcopters to show the improved performance of DTSA as compared to TDMA.

==> biblio.tex <==
@article{falconer1995time,
  title={Time division multiple access methods for wireless personal communications},
  author={Falconer, David D and Adachi, Fumiyuki and Gudmundson, Bjorn},
  journal={IEEE Communications Magazine},
  volume={33},
  number={1},
  pages={50--57},
  year={1995},
  publisher={IEEE}
}

@book{zigangirov2004theory,
  title={Theory of code division multiple access communication},
  author={Zigangirov, Kamil Sh},
  volume={6},
  year={2004},
  publisher={John Wiley \& Sons}
}

@inproceedings{sari1997analysis,
  title={An analysis of orthogonal frequency-division multiple access},
  author={Sari, Hikmet and Levy, Y and Karam, G},
  booktitle={GLOBECOM 97. IEEE Global Telecommunications Conference. Conference Record},
  volume={3},
  pages={1635--1639},
  year={1997},
  organization={IEEE}
}

@article{erdelj2017help,
  title={Help from the sky: Leveraging UAVs for disaster management},
  author={Erdelj, Milan and Natalizio, Enrico and Chowdhury, Kaushik R and Akyildiz, Ian F},
  journal={IEEE Pervasive Computing},
  volume={16},
  number={1},
  pages={24--32},
  year={2017},
  publisher={IEEE}
}

@INPROCEEDINGS{crazyflie,
  author={Giernacki, Wojciech and Skwierczyński, Mateusz and Witwicki, Wojciech and Wroński, Paweł and Kozierski, Piotr},
  booktitle={2017 22nd International Conference on Methods and Models in Automation and Robotics (MMAR)}, 
  title={Crazyflie 2.0 quadrotor as a platform for research and education in robotics and control engineering}, 
  year={2017},
  volume={},
  number={},
  pages={37-42},
  doi={10.1109/MMAR.2017.8046794}}
  
@article{radoglou2020compilation,
  title={A compilation of UAV applications for precision agriculture},
  author={Radoglou-Grammatikis, Panagiotis and Sarigiannidis, Panagiotis and Lagkas, Thomas and Moscholios, Ioannis},
  journal={Computer Networks},
  volume={172},
  pages={107148},
  year={2020},
  publisher={Elsevier}
}

@inproceedings{semsch2009autonomous,
  title={Autonomous UAV surveillance in complex urban environments},
  author={Semsch, Eduard and Jakob, Michal and Pavlicek, Du{\v{s}}an and Pechoucek, Michal},
  booktitle={2009 IEEE/WIC/ACM International Joint Conference on Web Intelligence and Intelligent Agent Technology},
  volume={2},
  pages={82--85},
  year={2009},
  organization={IEEE}
}

@misc{cr_comm,
  title = {Communication Protocols},
  howpublished = {\url{https://devzone.nordicsemi.com/f/nordic-q-a/66470/communication-protocols}},
  note = {last accessed: 04.11.2021}
}

@article{yasin2020unmanned,
  title={Unmanned aerial vehicles (uavs): Collision avoidance systems and approaches},
  author={Yasin, Jawad N and Mohamed, Sherif AS and Haghbayan, Mohammad-Hashem and Heikkonen, Jukka and Tenhunen, Hannu and Plosila, Juha},
  journal={IEEE Access},
  volume={8},
  pages={105139--105155},
  year={2020},
  publisher={IEEE}
}

@article{sharma2020communication,
  title={Communication and networking technologies for UAVs: A survey},
  author={Sharma, Abhishek and Vanjani, Pankhuri and Paliwal, Nikhil and Basnayaka, Chathuranga M Wijerathna and Jayakody, Dushantha Nalin K and Wang, Hwang-Cheng and Muthuchidambaranathan, P},
  journal={Journal of Network and Computer Applications},
  pages={102739},
  year={2020},
  publisher={Elsevier}
}

@misc{p2p_comm,
  title = {Bitcraze forum: Crazyflie communication between each other},
  howpublished = {\url{https://forum.bitcraze.io/viewtopic.php?t=4373\&hilit=p2p+multiple+\\crazyflies }},
  note = {last accessed: 04.11.2021}
}

@misc{pd3d,
  title = {Panda3D: The Open Source Framework for 3D Rendering and Games},
  howpublished = {\url{https://www.panda3d.org/}},
  note = {last accessed: 04.12.2021}
}

@INPROCEEDINGS{csma,
  author={Yun, Se-Young and Yi, Yung and Shin, Jinwoo and Eun, Do Young},
  booktitle={2012 IEEE International Conference on Communication Systems (ICCS)}, 
  title={Optimal CSMA: A survey}, 
  year={2012},
  volume={},
  number={},
  pages={199-204},
  doi={10.1109/ICCS.2012.6406138}}

==> control.tex <==




\usepackage{float}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{graphicx}
\graphicspath{{figures/}}
\usepackage{tikz}
% \usepackage{cases}
\usepackage{algpseudocode}
\usepackage{amsmath}
\usepackage{todonotes}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
% \usepackage{subfig}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{wrapfig}
% \usepackage{hyperref}


==> figures/ang1.tex <==
\begin{tikzpicture}
%%\node (a3) [fill=blue!50, circle, minimum size=1cm] at (50:7)  {$a_{3}$};



\node (a0) [circle, fill=blue!20, minimum size=2cm] at (0,0) {$a_{0}$};
\node (a1) [circle, fill=blue!20, minimum size=2cm] at (0:10cm) {$a_{1}$};
\node (v1) [->,red] at (40:2.6cm) {};




\draw[->, line width=0.1cm, black] (a0) --node[anchor=north]{$\textbf{p}_{0|1}$} (a1);
\draw[->, line width=0.1cm, red, anchor=west] (a0) --node[anchor=west]{$\textbf{v}_{0|1}$} (v1);

\coordinate (A) at (5cm,0);
\coordinate (B) at (0,0);
\coordinate (C) at (40:1cm);


\draw (A) -- (B) -- (C)
pic [draw=green!50!black, fill=green!20, angle, radius=9mm
"$70\%$"] {angle = A--B--C}; 40 deg = 70

\end{tikzpicture}


